A scalable parallel finite element framework for growing geometries. Application to metal additive manufacturing

This work introduces an innovative parallel, fully-distributed finite element framework for growing geometries and its application to metal additive manufacturing. It is well-known that virtual part design and qualification in additive manufacturing requires highly-accurate multiscale and multiphysics analyses. Only high performance computing tools are able to handle such complexity in time frames compatible with time-to-market. However, efficiency, without loss of accuracy, has rarely held the centre stage in the numerical community. Here, in contrast, the framework is designed to adequately exploit the resources of high-end distributed-memory machines. It is grounded on three building blocks: (1) Hierarchical adaptive mesh refinement with octree-based meshes; (2) a parallel strategy to model the growth of the geometry; (3) state-of-the-art parallel iterative linear solvers. Computational experiments consider the heat transfer analysis at the part scale of the printing process by powder-bed technologies. After verification against a 3D benchmark, a strong-scaling analysis assesses performance and identifies major sources of parallel overhead. A third numerical example examines the efficiency and robustness of (2) in a curved 3D shape. Unprecedented parallelism and scalability were achieved in this work. Hence, this framework contributes to take on higher complexity and/or accuracy, not only of part-scale simulations of metal or polymer additive manufacturing, but also in welding, sedimentation, atherosclerosis, or any other physical problem where the physical domain of interest grows in time.

==> Figures/application/DMLSBoundaryConditions.tex <==
\newcommand{\gear}[6]{%
  (0:#2)
  \foreach \i [evaluate=\i as \n using {\i-1)*360/#1}] in {1,...,#1}{%
    arc (\n:\n+#4:#2) {[rounded corners=1.5pt] -- (\n+#4+#5:#3)
    arc (\n+#4+#5:\n+360/#1-#5:#3)} --  (\n+360/#1:#2)
  }%
  (0,0) circle[radius=#6] 
}

\begin{tikzpicture}[scale = 1.0]
	
	\fill[fill=teal!40!white] (5, 2.5) -- (16, 2.5) -- (16, 6) -- (5, 6) -- cycle;
	\fill[fill=teal!80!white, even odd rule, xshift=10.5 cm, yshift=4.5cm] \gear{8}{1.7}{2}{20}{4}{1.0};
	
	\fill[fill=white] (9,6.0) rectangle (12,7.0);
	
	\filldraw[fill=gray!40!white, thin] (5, 2) -- node[very near start, below]{Building platform} (16, 2) -- (16, 2.5) -- node[white, very near end, above]{Powder bed} (5, 2.5) -- cycle;
	
	\draw[red!80!black, line width = 2.0pt] (9.2, 8) -- (9.2, 6);
    \draw[red!80!black, thick] (9.2, 6) -- (9.4, 6.3);
    \draw[red!80!black, thick] (8.9, 6.1) -- (9.2, 6) -- (9.5, 6.1);
    \draw[red!80!black, thick] (9.0, 6.3) -- (9.2, 6);
    
    \draw[ultra thick, ->] (8.8,6.2) sin (8.6,6.4) cos (8.4,6.6) sin (8.2,6.8) cos (8.0,7.0);
    \node[black, anchor=west] at (5.8,6.5) {Heat radiation}; 
    
    \draw[ultra thick, ->] (9.7,6.2) .. controls (10.5,6.2) .. (10.7,6.4);
    \draw[ultra thick, ->] (10.8,6.2) .. controls (11.6,6.2) .. (11.8,6.4);
    \node[black, anchor=west] at (9.7,6.8) {Heat convection}; 
    
    \draw[ultra thick, ->] (12,5) -- (12.65,5);
    \draw[ultra thick, ->] (12,4.5) -- (12.65,4.5);
    \draw[ultra thick, ->] (12,4) -- (12.65,4);
    
    \draw[ultra thick, ->] (9,5) -- (8.35,5);
    \draw[ultra thick, ->] (9,4.5) -- (8.35,4.5);
    \draw[ultra thick, ->] (9,4) -- (8.35,4);
    
    \node[black, anchor=west] at (12.75,4.5) {Heat conduction};
    
    \draw[ultra thick, ->] (9.8,2.75) -- (9.8,1.75);
    \draw[ultra thick, ->] (10.3,2.75) -- (10.3,1.75);
    
    \node[black, anchor=west] at (10.5,1.5) {Heat conduction};
    
	\node[teal!80!white, anchor=west] at (12,3) {Printed object}; 
			
\end{tikzpicture}

==> Figures/application/DMLSPrintingProcess.tex <==
% Gear macro
% #1 number of teeths
% #2 radius intern
% #3 radius extern
% #4 angle from start to end of the first arc
% #5 angle to decale the second arc from the first
% #6 inner radius to cut off
% #7 origin X
% #8 origin Y

\newcommand{\gear}[6]{%
  (0:#2)
  \foreach \i [evaluate=\i as \n using {\i-1)*360/#1}] in {1,...,#1}{%
    arc (\n:\n+#4:#2) {[rounded corners=1.5pt] -- (\n+#4+#5:#3)
    arc (\n+#4+#5:\n+360/#1-#5:#3)} --  (\n+360/#1:#2)
  }%
  (0,0) circle[radius=#6] 
}

\begin{tikzpicture}[scale = 1.0]
	
	\fill[fill=teal!40!white] (5, 2.5) -- (16, 2.5) -- (16, 6) -- (5, 6) -- cycle;
	\fill[fill=teal!40!white] (1, 3.5) -- (4, 3.5) -- (4, 6) -- (1, 6) -- cycle;
	\fill[fill=teal!40!white] (2.5, 5.3) -- (5, 5.3) .. controls (4.7, 6.3) .. (2.5, 6.3) -- cycle;
	
	\fill[fill=teal!80!white, even odd rule, xshift=10.5 cm, yshift=4.5cm] \gear{8}{1.7}{2}{20}{4}{1.0};
	
	\fill[fill=white] (9,6.0) rectangle (12,7.0);
	
	\filldraw[fill=gray!70!white, thin] (0, 0) -- (1, 0) -- (1, 6) -- (0, 6) -- cycle;
	\filldraw[fill=gray!70!white, thin] (4, 0) -- (5, 0) -- (5, 6) -- (4, 6) -- cycle;
	\filldraw[fill=gray!70!white, thin] (16, 0) -- (17, 0) -- (17, 6) -- (16, 6) -- cycle;
	
	\filldraw[fill=gray!40!white, thin] (1, 3) -- (4, 3) -- (4, 3.5) -- (1, 3.5) -- cycle;
	\filldraw[fill=gray!40!white, thin] (2.25, 0) -- (2.75, 0) -- (2.75, 3) -- (2.25, 3) -- cycle;
	\filldraw[fill=gray!40!white, thin] (10.25, 0) -- (10.75, 0) -- (10.75, 2) -- (10.25, 2) -- cycle;
	\filldraw[fill=gray!40!white, thin] (5, 2) -- node[near start, below = 0.5cm, font=\large]{Building platform} (16, 2) -- (16, 2.5) -- (5, 2.5) -- cycle;
	\filldraw[fill=gray!40!white, thin] (2, 6) -- (2.5, 6) -- (2.5, 8) -- node[above, font=\large]{Levelling blade} (2, 8) -- cycle;
	
	\draw[red!80!black, line width = 2.0pt] (9.2, 10) -- node[very near start,left,font=\large] {Laser} node[blue!60!black,left,font=\Large] {(2)} (9.2, 6);
    \draw[red!80!black, ultra thick] (9.2, 6) -- (9.4, 6.3);
    \draw[red!80!black, ultra thick] (8.9, 6.1) -- (9.2, 6) -- (9.5, 6.1);
    \draw[red!80!black, ultra thick] (9.0, 6.3) -- (9.2, 6);
    
    \draw[blue!60!black, line width = 4.0pt, ->] (3.15, 1) -- node[right,font=\Large] {(1)} (3.15, 2.5);
    \draw[blue!60!black, line width = 4.0pt, ->] (3, 7.0) -- node[above,font=\Large] {(1)} (4.5, 7.0);
    \draw[blue!60!black, line width = 4.0pt, ->] (11.15, 1.75) -- node[right,font=\Large] {(3)} (11.15, 0.25);
	
	\draw[blue!60!black, line width = 4.0pt, ->] (14,9) arc (90:200:1cm) node[left = 0.22cm, font=\Large]{(1)};
	\draw[blue!60!black, line width = 4.0pt, ->] (13.14,7.5) arc (210:320:1cm) node[below = 0.32cm, font=\Large]{(2)};
	\draw[blue!60!black, line width = 4.0pt, ->] (14.87,7.5) arc (-30:80:1cm) node[above = 0.25cm,right = 0.28cm, font=\Large]{(3)};
	\node[blue!60!black, font=\Large] at (14,8) {(4)};
	
	\node[white, font=\large, anchor=west] at (1.1,3.9) {Powder stock}; 
	\node[white, font=\large, anchor=west] at (5.1,2.9) {Powder bed}; 
	\node[teal!80!white, font=\large, anchor=west] at (12,3) {Printed object}; 
			
\end{tikzpicture}

==> Figures/parallel/subgraph-of-partition-0.tex <==
% Tikz File 'search-on-octree-0.tex'

\begin{tikzpicture}[font=\Huge]
    
    % Background mesh
	\node at (8,8) {\includegraphics[width=16cm,height=16cm]{figures/background-mesh}};
	   
    % Octree grid
    \draw[black, scale =  16] (0,0) grid (1,1);

\end{tikzpicture}

==> Figures/results/logPlots/coarse_dofs_max_degree.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{10}$}}}%
      \csname LTb\endcsname%
      \put(1210,1286){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{20}$}}}%
      \csname LTb\endcsname%
      \put(1210,1867){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{40}$}}}%
      \csname LTb\endcsname%
      \put(1210,2449){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{80}$}}}%
      \csname LTb\endcsname%
      \put(1210,3030){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{160}$}}}%
      \csname LTb\endcsname%
      \put(1210,3612){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{320}$}}}%
      \csname LTb\endcsname%
      \put(1210,4193){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{640}$}}}%
      \csname LTb\endcsname%
      \put(1210,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1280}$}}}%
      \csname LTb\endcsname%
      \put(1933,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(2805,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{192}$}}}%
      \csname LTb\endcsname%
      \put(3676,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{384}$}}}%
      \csname LTb\endcsname%
      \put(4548,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{768}$}}}%
      \csname LTb\endcsname%
      \put(5420,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{1536}$}}}%
      \csname LTb\endcsname%
      \put(6291,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{3072}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{$\max{\mathbf{n_{coarse \ dofs}}}$}}}}%
      \put(4072,154){\makebox(0,0){\strut{}\vspace{-0.2cm} \Large{Number of fine tasks}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{coarse_dofs_max_degree}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/coarse_dofs_max_dist.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{10}$}}}%
      \csname LTb\endcsname%
      \put(1210,1286){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{20}$}}}%
      \csname LTb\endcsname%
      \put(1210,1867){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{40}$}}}%
      \csname LTb\endcsname%
      \put(1210,2449){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{80}$}}}%
      \csname LTb\endcsname%
      \put(1210,3030){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{160}$}}}%
      \csname LTb\endcsname%
      \put(1210,3612){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{320}$}}}%
      \csname LTb\endcsname%
      \put(1210,4193){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{640}$}}}%
      \csname LTb\endcsname%
      \put(1210,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1280}$}}}%
      \csname LTb\endcsname%
      \put(1933,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(2805,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{192}$}}}%
      \csname LTb\endcsname%
      \put(3676,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{384}$}}}%
      \csname LTb\endcsname%
      \put(4548,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{768}$}}}%
      \csname LTb\endcsname%
      \put(5420,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{1536}$}}}%
      \csname LTb\endcsname%
      \put(6291,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{3072}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{$\max\left(\mathbf{n_{coarse \ dofs}}\right)$}}}}%
      \put(4072,154){\makebox(0,0){\strut{}\vspace{-0.2cm} \Large{Number of fine tasks}}}%
      \csname LTb\endcsname%
      \put(5816,1537){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 1}$}}}%
      \csname LTb\endcsname%
      \put(5816,1317){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 2}$}}}%
      \csname LTb\endcsname%
      \put(5816,1097){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 3}$}}}%
      \csname LTb\endcsname%
      \put(5816,877){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 4}$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{coarse_dofs_max_dist}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/coarse_problem_mean.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{128}$}}}%
      \csname LTb\endcsname%
      \put(1342,1213){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{256}$}}}%
      \csname LTb\endcsname%
      \put(1342,1722){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{512}$}}}%
      \csname LTb\endcsname%
      \put(1342,2231){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1024}$}}}%
      \csname LTb\endcsname%
      \put(1342,2740){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{2048}$}}}%
      \csname LTb\endcsname%
      \put(1342,3248){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{4096}$}}}%
      \csname LTb\endcsname%
      \put(1342,3757){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{8192}$}}}%
      \csname LTb\endcsname%
      \put(1342,4266){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{16384}$}}}%
      \csname LTb\endcsname%
      \put(1342,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{32768}$}}}%
      \csname LTb\endcsname%
      \put(1972,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(2705,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{192}$}}}%
      \csname LTb\endcsname%
      \put(3439,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{384}$}}}%
      \csname LTb\endcsname%
      \put(4173,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{768}$}}}%
      \csname LTb\endcsname%
      \put(4906,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{1536}$}}}%
      \csname LTb\endcsname%
      \put(5640,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{3072}$}}}%
      \csname LTb\endcsname%
      \put(6374,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{6144}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Mean coarse DOFs}}}}%
      \put(4138,154){\makebox(0,0){\strut{}\vspace{-0.2cm} \Large{Number of fine tasks}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{coarse_problem_mean}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/dofs_partition_weights.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{0.2}$}}}%
      \csname LTb\endcsname%
      \put(1078,1518){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{0.4}$}}}%
      \csname LTb\endcsname%
      \put(1078,2332){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{0.8}$}}}%
      \csname LTb\endcsname%
      \put(1078,3147){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1.6}$}}}%
      \csname LTb\endcsname%
      \put(1078,3961){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{3.2}$}}}%
      \csname LTb\endcsname%
      \put(1078,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{6.4}$}}}%
      \csname LTb\endcsname%
      \put(1815,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(2708,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{192}$}}}%
      \csname LTb\endcsname%
      \put(3601,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{384}$}}}%
      \csname LTb\endcsname%
      \put(4494,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{768}$}}}%
      \csname LTb\endcsname%
      \put(5386,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{1536}$}}}%
      \csname LTb\endcsname%
      \put(6279,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{3072}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Interprocessor variability $\boldsymbol{\mu(c_v^p)}$}}}}%
      \put(4006,154){\makebox(0,0){\strut{}\vspace{-0.2cm} \Large{Number of fine tasks}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{dofs_partition_weights}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/iterations_max_dist.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{24}$}}}%
      \csname LTb\endcsname%
      \put(946,2740){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{48}$}}}%
      \csname LTb\endcsname%
      \put(946,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(1698,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(2611,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{192}$}}}%
      \csname LTb\endcsname%
      \put(3525,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{384}$}}}%
      \csname LTb\endcsname%
      \put(4439,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{768}$}}}%
      \csname LTb\endcsname%
      \put(5353,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{1536}$}}}%
      \csname LTb\endcsname%
      \put(6267,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{3072}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{PCG iterations}}}}%
      \put(3940,154){\makebox(0,0){\strut{}\vspace{-0.2cm} \Large{Number of fine tasks}}}%
      \csname LTb\endcsname%
      \put(1698,1270){\makebox(0,0){\strut{}27}}%
      \put(2611,1676){\makebox(0,0){\strut{}31}}%
      \put(3525,2350){\makebox(0,0){\strut{}39}}%
      \put(4439,3020){\makebox(0,0){\strut{}49}}%
      \put(5353,3758){\makebox(0,0){\strut{}63}}%
      \put(6267,4385){\makebox(0,0){\strut{}78}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{iterations_max_dist}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/iterations_mean.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{24}$}}}%
      \csname LTb\endcsname%
      \put(946,2740){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{48}$}}}%
      \csname LTb\endcsname%
      \put(946,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(1698,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(2611,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{192}$}}}%
      \csname LTb\endcsname%
      \put(3525,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{384}$}}}%
      \csname LTb\endcsname%
      \put(4439,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{768}$}}}%
      \csname LTb\endcsname%
      \put(5353,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{1536}$}}}%
      \csname LTb\endcsname%
      \put(6267,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{3072}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Mean PCG iterations}}}}%
      \put(3940,154){\makebox(0,0){\strut{}\vspace{-0.2cm} \Large{Num fine tasks}}}%
      \csname LTb\endcsname%
      \put(1698,1270){\makebox(0,0){\strut{}27}}%
      \put(2611,1676){\makebox(0,0){\strut{}31}}%
      \put(3525,2350){\makebox(0,0){\strut{}39}}%
      \put(4439,3020){\makebox(0,0){\strut{}49}}%
      \put(5353,3758){\makebox(0,0){\strut{}63}}%
      \put(6267,4385){\makebox(0,0){\strut{}78}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{iterations_mean}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/iterations_partition_weights.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{12}$}}}%
      \csname LTb\endcsname%
      \put(946,2061){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{24}$}}}%
      \csname LTb\endcsname%
      \put(946,3418){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{48}$}}}%
      \csname LTb\endcsname%
      \put(946,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(1698,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{96}$}}}%
      \csname LTb\endcsname%
      \put(2611,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{192}$}}}%
      \csname LTb\endcsname%
      \put(3525,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{384}$}}}%
      \csname LTb\endcsname%
      \put(4439,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{768}$}}}%
      \csname LTb\endcsname%
      \put(5353,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{1536}$}}}%
      \csname LTb\endcsname%
      \put(6267,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{3072}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Mean PCG iterations}}}}%
      \put(3940,154){\makebox(0,0){\strut{}\vspace{-0.2cm} \Large{Num fine tasks}}}%
      \csname LTb\endcsname%
      \put(5816,1537){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 1}$}}}%
      \csname LTb\endcsname%
      \put(5816,1317){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 10}$}}}%
      \csname LTb\endcsname%
      \put(5816,1097){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 100}$}}}%
      \csname LTb\endcsname%
      \put(5816,877){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = \infty}$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{iterations_partition_weights}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScaling.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,1929){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,2646){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(682,3155){\makebox(0,0)[r]{\strut{}$4$}}%
      \put(682,3550){\makebox(0,0)[r]{\strut{}$5$}}%
      \put(682,3872){\makebox(0,0)[r]{\strut{}$6$}}%
      \put(682,4144){\makebox(0,0)[r]{\strut{}$7$}}%
      \put(682,4380){\makebox(0,0)[r]{\strut{}$8$}}%
      \put(682,4589){\makebox(0,0)[r]{\strut{}$9$}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(814,484){\makebox(0,0){\strut{}$10$}}%
      \put(2815,484){\makebox(0,0){\strut{}$100$}}%
      \put(4816,484){\makebox(0,0){\strut{}$1000$}}%
      \put(5923,968){\makebox(0,0)[l]{\strut{}$100$}}%
      \put(5923,3691){\makebox(0,0)[l]{\strut{}$1000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Speed-up}}}%
      \put(6692,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Total wall time [s]}}}%
      \put(3302,154){\makebox(0,0){\strut{}Number of cores}}%
      \csname LTb\endcsname%
      \put(4804,1317){\makebox(0,0)[r]{\strut{}Speed-up}}%
      \csname LTb\endcsname%
      \put(4804,1097){\makebox(0,0)[r]{\strut{}Wall time}}%
      \csname LTb\endcsname%
      \put(4804,877){\makebox(0,0)[r]{\strut{}Ideal}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScaling}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingMaxDegree.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{200}$}}}%
      \csname LTb\endcsname%
      \put(1210,1581){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{400}$}}}%
      \csname LTb\endcsname%
      \put(1210,2739){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1000}$}}}%
      \csname LTb\endcsname%
      \put(1210,3616){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{2000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4129){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{3000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4493){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{4000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{5000}$}}}%
      \csname LTb\endcsname%
      \put(1342,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(3162,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4983,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Total wall time [s]}}}}%
      \put(4072,154){\makebox(0,0){\strut{}\Large{Number of fine tasks}}}%
      \csname LTb\endcsname%
      \put(2662,1537){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{\Delta^{\max} = 10}$}}}%
      \csname LTb\endcsname%
      \put(2662,1317){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{\Delta^{\max} = 20}$}}}%
      \csname LTb\endcsname%
      \put(2662,1097){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{\Delta^{\max} = 50}$}}}%
      \csname LTb\endcsname%
      \put(2662,877){\makebox(0,0)[r]{\strut{}\Large{Ideal}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingMaxDegree}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingMaxDegreeFraction.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{80}$}}}%
      \csname LTb\endcsname%
      \put(1078,1722){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{100}$}}}%
      \csname LTb\endcsname%
      \put(1078,2740){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{120}$}}}%
      \csname LTb\endcsname%
      \put(1078,3757){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{140}$}}}%
      \csname LTb\endcsname%
      \put(1078,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{160}$}}}%
      \csname LTb\endcsname%
      \put(1210,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(3074,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4939,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Total wall time w.r.t. BDDC-ref [\%]}}}}%
      \put(4006,154){\makebox(0,0){\strut{}\Large{Number of fine tasks}}}%
      \csname LTb\endcsname%
      \put(2530,4602){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{\Delta^{\max} = 10}$}}}%
      \csname LTb\endcsname%
      \put(2530,4382){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{\Delta^{\max} = 20}$}}}%
      \csname LTb\endcsname%
      \put(2530,4162){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{\Delta^{\max} = 50}$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingMaxDegreeFraction}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingMaxDist.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{200}$}}}%
      \csname LTb\endcsname%
      \put(1210,1581){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{400}$}}}%
      \csname LTb\endcsname%
      \put(1210,2739){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1000}$}}}%
      \csname LTb\endcsname%
      \put(1210,3616){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{2000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4129){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{3000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4493){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{4000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{5000}$}}}%
      \csname LTb\endcsname%
      \put(1342,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(3162,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4983,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Total wall time [s]}}}}%
      \put(4072,154){\makebox(0,0){\strut{}\Large{Number of fine tasks}}}%
      \csname LTb\endcsname%
      \put(2530,1757){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 1}$}}}%
      \csname LTb\endcsname%
      \put(2530,1537){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 2}$}}}%
      \csname LTb\endcsname%
      \put(2530,1317){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 3}$}}}%
      \csname LTb\endcsname%
      \put(2530,1097){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 4}$}}}%
      \csname LTb\endcsname%
      \put(2530,877){\makebox(0,0)[r]{\strut{}\Large{Ideal}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingMaxDist}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingMaxDistFraction.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{60}$}}}%
      \csname LTb\endcsname%
      \put(1078,2061){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{80}$}}}%
      \csname LTb\endcsname%
      \put(1078,3418){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{100}$}}}%
      \csname LTb\endcsname%
      \put(1078,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{120}$}}}%
      \csname LTb\endcsname%
      \put(1210,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(3074,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4939,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Total wall time w.r.t. BDDC-ref [\%]}}}}%
      \put(4006,154){\makebox(0,0){\strut{}\Large{Number of fine tasks}}}%
      \csname LTb\endcsname%
      \put(2398,4602){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 1}$}}}%
      \csname LTb\endcsname%
      \put(2398,4382){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 2}$}}}%
      \csname LTb\endcsname%
      \put(2398,4162){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 3}$}}}%
      \csname LTb\endcsname%
      \put(2398,3942){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{d^{\max} = 4}$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingMaxDistFraction}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingPartitionWeights.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{200}$}}}%
      \csname LTb\endcsname%
      \put(1210,1581){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{400}$}}}%
      \csname LTb\endcsname%
      \put(1210,2739){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1000}$}}}%
      \csname LTb\endcsname%
      \put(1210,3616){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{2000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4129){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{3000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4493){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{4000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{5000}$}}}%
      \csname LTb\endcsname%
      \put(1342,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(3162,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4983,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Total wall time [s]}}}}%
      \put(4072,154){\makebox(0,0){\strut{}\Large{Number of fine tasks}}}%
      \csname LTb\endcsname%
      \put(3190,1757){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 1}$}}}%
      \csname LTb\endcsname%
      \put(3190,1537){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 10}$}}}%
      \csname LTb\endcsname%
      \put(3190,1317){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 100}$}}}%
      \csname LTb\endcsname%
      \put(3190,1097){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = \infty}$}}}%
      \csname LTb\endcsname%
      \put(3190,877){\makebox(0,0)[r]{\strut{}\Large{Ideal}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingPartitionWeights}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingPartitionWeightsFraction.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{50}$}}}%
      \csname LTb\endcsname%
      \put(1078,1722){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{100}$}}}%
      \csname LTb\endcsname%
      \put(1078,2740){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{150}$}}}%
      \csname LTb\endcsname%
      \put(1078,3757){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{200}$}}}%
      \csname LTb\endcsname%
      \put(1078,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{250}$}}}%
      \csname LTb\endcsname%
      \put(1210,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(3074,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4939,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Total wall time w.r.t. BDDC-ref [\%]}}}}%
      \put(4006,154){\makebox(0,0){\strut{}\Large{Number of fine tasks}}}%
      \csname LTb\endcsname%
      \put(3058,4602){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 1}$}}}%
      \csname LTb\endcsname%
      \put(3058,4382){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 2}$}}}%
      \csname LTb\endcsname%
      \put(3058,4162){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 4}$}}}%
      \csname LTb\endcsname%
      \put(3058,3942){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 10}$}}}%
      \csname LTb\endcsname%
      \put(3058,3722){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = 100}$}}}%
      \csname LTb\endcsname%
      \put(3058,3502){\makebox(0,0)[r]{\strut{}\Large{$\mathbf{w_a/w_i = \infty}$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingPartitionWeightsFraction}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingPercentagePhases.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{0}$}}}%
      \csname LTb\endcsname%
      \put(1078,1111){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{10}$}}}%
      \csname LTb\endcsname%
      \put(1078,1518){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{20}$}}}%
      \csname LTb\endcsname%
      \put(1078,1925){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{30}$}}}%
      \csname LTb\endcsname%
      \put(1078,2332){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{40}$}}}%
      \csname LTb\endcsname%
      \put(1078,2740){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{50}$}}}%
      \csname LTb\endcsname%
      \put(1078,3147){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{60}$}}}%
      \csname LTb\endcsname%
      \put(1078,3554){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{70}$}}}%
      \csname LTb\endcsname%
      \put(1078,3961){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{80}$}}}%
      \csname LTb\endcsname%
      \put(1078,4368){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{90}$}}}%
      \csname LTb\endcsname%
      \put(1078,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{100}$}}}%
      \csname LTb\endcsname%
      \put(1210,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(3074,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4939,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Fraction of total wall time [\%]}}}}%
      \put(4006,154){\makebox(0,0){\strut{}\Large{Number of subdomains}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingPercentagePhases}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingPoisson.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1}$}}}%
      \csname LTb\endcsname%
      \put(946,1534){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{2}$}}}%
      \csname LTb\endcsname%
      \put(946,2363){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{4}$}}}%
      \csname LTb\endcsname%
      \put(946,2849){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{6}$}}}%
      \csname LTb\endcsname%
      \put(946,3460){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{10}$}}}%
      \csname LTb\endcsname%
      \put(946,4290){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{20}$}}}%
      \csname LTb\endcsname%
      \put(946,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{30}$}}}%
      \csname LTb\endcsname%
      \put(1078,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(2986,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4895,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Speed-up}}}}%
      \put(3940,154){\makebox(0,0){\strut{}\Large{Number of fine tasks}}}%
      \csname LTb\endcsname%
      \put(5816,1317){\makebox(0,0)[r]{\strut{}\Large{AM BDDC-ref}}}%
      \csname LTb\endcsname%
      \put(5816,1097){\makebox(0,0)[r]{\strut{}\Large{Poisson BDDC-f}}}%
      \csname LTb\endcsname%
      \put(5816,877){\makebox(0,0)[r]{\strut{}\Large{Ideal}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingPoisson}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingSpeedUp.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1}$}}}%
      \csname LTb\endcsname%
      \put(946,1929){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{2}$}}}%
      \csname LTb\endcsname%
      \put(946,2646){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{3}$}}}%
      \csname LTb\endcsname%
      \put(946,3155){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{4}$}}}%
      \csname LTb\endcsname%
      \put(946,3550){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{5}$}}}%
      \csname LTb\endcsname%
      \put(946,3872){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{6}$}}}%
      \csname LTb\endcsname%
      \put(946,4144){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{7}$}}}%
      \csname LTb\endcsname%
      \put(946,4380){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{8}$}}}%
      \csname LTb\endcsname%
      \put(946,4589){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{9}$}}}%
      \csname LTb\endcsname%
      \put(946,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{10}$}}}%
      \csname LTb\endcsname%
      \put(1078,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(2986,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4895,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Speed-up}}}}%
      \put(3940,154){\makebox(0,0){\strut{}\Large{Number of subdomains}}}%
      \csname LTb\endcsname%
      \put(5816,1317){\makebox(0,0)[r]{\strut{}\Large{PCG-BDDC-ref}}}%
      \csname LTb\endcsname%
      \put(5816,1097){\makebox(0,0)[r]{\strut{}\Large{CG}}}%
      \csname LTb\endcsname%
      \put(5816,877){\makebox(0,0)[r]{\strut{}\Large{Ideal}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingSpeedUp}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingSpeedUpPhases.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1}$}}}%
      \csname LTb\endcsname%
      \put(946,1534){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{2}$}}}%
      \csname LTb\endcsname%
      \put(946,2019){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{3}$}}}%
      \csname LTb\endcsname%
      \put(946,2363){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{4}$}}}%
      \csname LTb\endcsname%
      \put(946,2630){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{5}$}}}%
      \csname LTb\endcsname%
      \put(946,2849){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{6}$}}}%
      \csname LTb\endcsname%
      \put(946,3193){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{8}$}}}%
      \csname LTb\endcsname%
      \put(946,3460){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{10}$}}}%
      \csname LTb\endcsname%
      \put(946,4290){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{20}$}}}%
      \csname LTb\endcsname%
      \put(946,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{30}$}}}%
      \csname LTb\endcsname%
      \put(1078,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(2986,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4895,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Speed-up}}}}%
      \put(3940,154){\makebox(0,0){\strut{}\Large{Number of subdomains}}}%
      \csname LTb\endcsname%
      \put(3454,4602){\makebox(0,0)[r]{\strut{}\Large{Total simulation}}}%
      \csname LTb\endcsname%
      \put(3454,4382){\makebox(0,0)[r]{\strut{}\Large{Triangulation}}}%
      \csname LTb\endcsname%
      \put(3454,4162){\makebox(0,0)[r]{\strut{}\Large{Activation}}}%
      \csname LTb\endcsname%
      \put(3454,3942){\makebox(0,0)[r]{\strut{}\Large{Assembly}}}%
      \csname LTb\endcsname%
      \put(3454,3722){\makebox(0,0)[r]{\strut{}\Large{Solver}}}%
      \csname LTb\endcsname%
      \put(3454,3502){\makebox(0,0)[r]{\strut{}\Large{Ideal}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingSpeedUpPhases}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/results/logPlots/strongScalingWallTime.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\bfseries
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,704){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{200}$}}}%
      \csname LTb\endcsname%
      \put(1210,1581){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{400}$}}}%
      \csname LTb\endcsname%
      \put(1210,2739){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{1000}$}}}%
      \csname LTb\endcsname%
      \put(1210,3616){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{2000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4129){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{3000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4493){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{4000}$}}}%
      \csname LTb\endcsname%
      \put(1210,4775){\makebox(0,0)[r]{\strut{}\Large{$\boldsymbol{5000}$}}}%
      \csname LTb\endcsname%
      \put(1342,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{1}}$}}}%
      \csname LTb\endcsname%
      \put(3162,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{2}}$}}}%
      \csname LTb\endcsname%
      \put(4983,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{3}}$}}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}\Large{$\boldsymbol{10^{4}}$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}\vspace{-1.0cm} \Large{Total wall time [s]}}}}%
      \put(4072,154){\makebox(0,0){\strut{}\Large{Number of subdomains}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{strongScalingWallTime}}%
    \gplfronttext
  \end{picture}%
\endgroup

